Challenging Machine Learning-based Clone Detectors via Semantic-preserving Code Transformations

Software clone detection identifies similar code snippets. It has been an active research topic that attracts extensive attention over the last two decades. In recent years, machine learning (ML) based detectors, especially deep learning-based ones, have demonstrated impressive capability on clone detection. It seems that this longstanding problem has already been tamed owing to the advances in ML techniques. In this work, we would like to challenge the robustness of the recent ML-based clone detectors through code semantic-preserving transformations. We first utilize fifteen simple code transformation operators combined with commonly-used heuristics (i.e., Random Search, Genetic Algorithm, and Markov Chain Monte Carlo) to perform equivalent program transformation. Furthermore, we propose a deep reinforcement learning-based sequence generation (DRLSG) strategy to effectively guide the search process of generating clones that could escape from the detection. We then evaluate the ML-based detectors with the pairs of original and generated clones. We realize our method in a framework named CloneGen. CloneGen In evaluation, we challenge the two state-of-the-art ML-based detectors and four traditional detectors with the code clones after semantic-preserving transformations via the aid of CloneGen. Surprisingly, our experiments show that, despite the notable successes achieved by existing clone detectors, the ML models inside these detectors still cannot distinguish numerous clones produced by the code transformations in CloneGen. In addition, adversarial training of ML-based clone detectors using clones generated by CloneGen can improve their robustness and accuracy. CloneGen Meanwhile, compared with the commonly-used heuristics, the DRLSG strategy has shown the best effectiveness in generating code clones to decrease the detection accuracy of the ML-based detectors.

==> CompareToobfuscator.tex <==
\lstset{
		frame=single, 
		language=c++,
		backgroundcolor=\color{white},
		extendedchars=true,
		%basicstyle=\fontsize{7}{7}\linespread{0.8}\selectfont\ttfamily,%\footnotesize\ttfamily,
		basicstyle=\scriptsize,
% 		showstringspaces=false,
% 		showspaces=false,
		numbers=left,
		numberstyle=\tiny\color{gray},
		numberstyle=\color{gray},
		keywordstyle=\color{blue}, 
		numbersep=5pt,
		xleftmargin=.25in,
% 		tabsize=2,
		breaklines=true,
% 		showtabs=false,
		captionpos=b,
		keepspaces=true,
		stepnumber=1,
% 		column=flexible,
		aboveskip=2mm,
		belowskip=2mm
}

\begin{figure}[!ht]
\footnotesize
% \vspace{-4mm}
\begin{minipage}[t]{0.49\linewidth} 
\centering      
\begin{lstlisting}  
// #1 Code 1
s=0;
for(i=1;i<=100;i++){
   s+=i;}
// #2 Mutated code
s=0;i=1;
while(i<=100){
   s+=i;i++;}
//#3 Obfuscating  via 
//control flow flattening
int swVar=1;
while(swVar!=0){
  switch(swVar){
  case 1:{i=1;s=0;swvar=2;break;
  }case 2:{if(i<=10) swVar=3;
  else swVar=0; break;
  }case 3:{s+=i;i++;
    swVar=2;break;
}}}
\end{lstlisting} 
\end{minipage}
\begin{minipage}[t]{0.49\linewidth} 
\centering 
\begin{lstlisting} 
// #4 Code 2
int main() {
  int i = 1;while(i <= 100) {
    if(i % 15 == 0)
      puts("FizzBuzz");
    else if(i % 5 == 0)
      puts("Buzz");
    else  printf("%d\n", i);
    i++;}}
// #5 Mutated via RM
int main () {
  int i1 = 1;
  for (; 100 >= i1;) {
    if (!(0 != i1 % 15))
      puts ("FizzBuzz");
    else {if (i1 % 5 == 0)
          puts ("Buzz");
          else;};}
    i1++;};}
\end{lstlisting} 
\end{minipage}
 

\begin{minipage}[t]{\linewidth}      
\centering       
\begin{lstlisting}  
 // #6 Obfuscating via code encoding
int main(){int o_8ffc9af5e5913588bc0b7705602caf02=(0x0000000000000002 + 0x0000000000000201 + 0x0000000000000801 - 0x0000000000000A03);while ((o_8ffc9af5e5913588bc0b7705602caf02 <= (0x00000000000000C8 + 0x0000000000000264 + 0x0000000000000864 - 0x0000000000000B2C)) & !!(o_8ffc9af5e5913588bc0b7705602caf02 <= (0x00000000000000C8 + 0x0000000000000264 + 0x0000000000000864 - 0x0000000000000B2C))){if (!(o_8ffc9af5e5913588bc0b7705602caf02 % (0x000000000000001E + 0x000000000000020F + 0x000000000000080F - 0x0000000000000A2D) ^ 0x0000000000000000))puts("\x46""i\172z\x42""u\172z");else if (!(o_8ffc9af5e5913588bc0b7705602caf02 % (0x000000000000000A + 0x0000000000000205 + 0x0000000000000805 - 0x0000000000000A0F) ^ 0x0000000000000000))puts("\x42""u\172z");else printf("\x25""d\012",o_8ffc9af5e5913588bc0b7705602caf02);;;
;o_8ffc9af5e5913588bc0b7705602caf02++;};};
\end{lstlisting}   
\end{minipage}
% \vspace{-4mm}
\caption{Mutation vs Obfuscation} 
\label{fig:obfuscatro}
% \vspace{-5mm}
\end{figure}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> dlMutatedSelected.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \footnotesize
  \centering
  \caption{The F1 results of TokenLSTM with adversarial training under different strategies}
    \setlength{\tabcolsep}{1.2mm}
    \begin{tabular}{l|ccccc}
    \toprule
    \diagbox{TestData}{$F_1$}{TrainData} & $D_I$ & 
   \multicolumn{1}{p{3.835em}}{$D_I$+\newline{}$D_{RS}^\prime$} & \multicolumn{1}{p{4.055em}}{$D_I$+\newline{}$D_{GA}^\prime$} & \multicolumn{1}{p{4.055em}}{$D_I$+\newline{}$D_{MCMC}^\prime$} & \multicolumn{1}{p{4.055em}}{$D_I$+\newline{}$D_{DRL}^\prime$}  \\
    \midrule
    $D_I$ & 0.991 & \textbf{0.997} & 0.989 & 0.992 & 0.993 \\
    $D_{RS}$ & 0.797 & \textbf{0.993} & 0.977 & 0.980  &  0.990 \\
    $D_{GA}$ & 0.613 & \textbf{0.979} & 0.974 & 0.957 & 0.972 \\
    $D_{MCMC}$ & 0.785 & \textbf{0.992} & 0.981 & 0.988 & 0.989 \\
    $D_{DRL}$ & 0.421 & 0.976 & \textbf{0.988} & 0.961 & 0.985 \\
    \bottomrule
    \end{tabular}%
  \label{tab:mutated_selec}%
\end{table}%

% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{lccccc}
%     \toprule
%     \multicolumn{1}{p{4.5em}}{TrainData      
%     \newline{}$F_1$\newline{}TestData} & $D_I$ & 
%     \multicolumn{1}{p{3.835em}}{$D_I$+\newline{}$D_{RS}^\prime$} & \multicolumn{1}{p{4.055em}}{$D_I$+\newline{}$D_{GA}^\prime$} & \multicolumn{1}{p{4.055em}}{$D_I$+\newline{}$D_{MCMC}^\prime$} & \multicolumn{1}{p{4.055em}}{$D_I$+\newline{}$D_{DRL}^\prime$} \\
%     \midrule
%     $D_I$ & 0.991 & \textbf{0.997} & 0.989 & 0.992 & 0.993 \\
%     $D_{RS}$ & 0.797 & \textbf{0.993} & 0.977 & 0.98  & 0.946 \\
%     $D_{GA}$ & 0.613 & \textbf{0.979} & 0.974 & 0.957 & 0.883 \\
%     $D_{MCMC}$ & 0.785 & \textbf{0.992} & 0.981 & 0.988 & 0.954 \\
%     $D_{DRL}$ & 0.421 & 0.976 & 0.988 & 0.961 & 0.985 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%



% \begin{table}[t]
% 	\footnotesize
% 	\caption{The F1 results of TokenLSTM with adversarial training under different strategies}
% 	\vspace{-2mm}
% 	\label{tab:mutated_selec}
% 	\setlength{\tabcolsep}{2.1mm}{
% \begin{tabular}{@{}p{1.5cm}p{1.05cm}p{1.05cm}p{1.05cm}p{1.05cm}p{1.05cm}@{}}
% \toprule 
%  \multicolumn{1}{l}{{\color[HTML]{000000} F1}} &
%  \multicolumn{1}{l}{{\color[HTML]{000000} Original}} &
%   \multicolumn{1}{l}{{\color[HTML]{000000} RM}} &
%   \multicolumn{1}{l}{{\color[HTML]{000000} GA}} &
%   \multicolumn{1}{l}{{\color[HTML]{000000} MCMC}} &
%   \multicolumn{1}{l}{{\color[HTML]{000000} DRLSG}} \\ \midrule
% {\color[HTML]{000000} Original} &
%   {\color[HTML]{000000} 0.991} &
%   {\color[HTML]{000000} 0.797} &
%   {\color[HTML]{000000} 0.613} &
%   {\color[HTML]{000000} 0.785} &
%   {\color[HTML]{000000} 0.421} \\
% {\color[HTML]{000000} RS\_Add} &
%   {\color[HTML]{000000} \textbf{0.997}} &
%   {\color[HTML]{000000} \textbf{0.993}} &
%   {\color[HTML]{000000} \textbf{0.979}} &
%   {\color[HTML]{000000} \textbf{0.992}} &
%   {\color[HTML]{000000} 0.976} \\
% {\color[HTML]{000000} GA\_Add} &
%   {\color[HTML]{000000} 0.989} &
%   {\color[HTML]{000000} 0.977} &
%   {\color[HTML]{000000} 0.974} &
%   {\color[HTML]{000000} 0.981} &
%   {\color[HTML]{000000} 0.961} \\
% {\color[HTML]{000000} MCMC\_Add} &
%   {\color[HTML]{000000} 0.992} &
%   {\color[HTML]{000000} 0.980} &
%   {\color[HTML]{000000} 0.957} &
%   {\color[HTML]{000000} 0.988} &
%   {\color[HTML]{000000} 0.961} \\
% {\color[HTML]{000000} DRLSG\_ADD} &
%   {\color[HTML]{000000} 0.993} &
%   {\color[HTML]{000000} 0.946} &
%   {\color[HTML]{000000} 0.883} &
%   {\color[HTML]{000000} 0.954} &
%   {\color[HTML]{000000} \textbf{0.985}} \\ \bottomrule
% \end{tabular}
% }
% \vspace{-2mm}
% \end{table}

==> dlPerformanceInPaper.tex <==
% \begin{table}[htpb]
%     \centering
%   \begin{tabular}{cccc}
% \toprule
% Tools          &P &  R &F1  \\
% \midrule
% \Astnn &0.98  &0.92&  0.95    \\
% \TBCCD   &0.99  & 0.99 & 0.99 \\
% \FCDector & 0.97  &0.95 &   0.96 \\
% \bottomrule
% \end{tabular}
%     \caption{Deep learning method for source code clone detection performance on OJClone data. These data are taken from the corresponding paper.\hy{can combine Table 5 and 7}
% }
%     \label{tab:toos_performance}
% \centering
% \end{table}

\begin{table}[t]
\footnotesize
\caption{ML-based detectors performance on OJClone}
% \vspace{-2mm}
\label{tab:toos_performance}
\centering
\begin{tabular}{p{1.25cm}cccccc}
\toprule
\multicolumn{1}{c}{}                   & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Original Performance\end{tabular}} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}New Performance\end{tabular}} \\ 
\cline{2-7} 
\multicolumn{1}{c}{\multirow{-2}{*}{}} & $P$ & $R$ & $F_1$    & $P$    & $R$  & $F_1$         \\ 
\midrule
\Astnn           & 0.98\%      & 0.92\%      & 0.95\%      & \textbf{0.99\%}& \textbf{0.97\%}  & \textbf{0.98\%}  \\
\TBCCD           & 0.99\%      & 0.99\%      &  0.99\%     & \textbf{1.00\%}   & 0.98\%   & 0.99\%                   \\
\FCDector      & 0.97 \%     & 0.95\%      & 0.96\%      & 0.97\%  & \textbf{0.97\%}  & \textbf{0.97\%}         \\ 
\bottomrule
\end{tabular}
\centering
% \vspace{-2mm}
\end{table}


==> lineofCode.tex <==
\begin{table}[t]
\footnotesize
\caption{The change in the number of lines after mutation}
\label{tab:lineofCode}
% \vspace{-2mm}
\centering
\begin{tabular}{p{1.85cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}}
\toprule
 & AM & RM  & GA & MCMC    \\
\midrule
\# Lines Before    & 366204  & 366227 & 366023 & 366277 \\
\# Lines After      & 1073970   & 634119   &  769677  & 559039  \\   
\# Growth rates     & 2.93    & 1.73      &  2.10    &   1.53\\
\bottomrule
\end{tabular}
% \vspace{-4mm}
\centering
\end{table}

==> tokenRepresentation.tex <==
\begin{figure}[!htbp]
	\centering
	\begin{subfigure}[b]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./tokenLSTM.png}
		\caption{TokenLSTM embedding}
		\label{fig:a}
	\end{subfigure}
	\begin{subfigure}[b]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./tokenDpcnn.png}
		\caption{TokenDPCNN embedding}
		\label{fig:b}
	\end{subfigure}
	\vspace{-4mm}
	\caption{The Code embedding representation}
	\label{fig:codeEmbedding}
	\vspace{-2mm}
\end{figure}


==> toolandItsMethods.tex <==
\begin{table}[t]   
\footnotesize
\caption{The ML-based detectors, the features and models}    
% \vspace{-2mm}
\label{tab:toolAttrModel} 
\centering
\begin{tabular}{p{2.2cm}p{2cm}p{3.4cm}}
\toprule
Tools      & Feature & DL Model            \\ 
\midrule
\Astnn      & AST       & Bidirectional GRU  \\
\TBCCD      & AST       & Tree-Base Convolution \\
\FCDector & AST, CFG   & Feedforward Neural Network \\ 
\bottomrule
\end{tabular}    
% \vspace{-4mm}
\centering 
\end{table}
